Validating and describing linked data portals using shapes

Linked data portals need to be able to advertise and describe the structure of their content. A sufficiently expressive and intuitive schema language will allow portals to communicate these structures. Validation tools will aid in the publication and maintenance of linked data and increase their quality. Two schema language proposals have recently emerged for describing the structures of RDF graphs: Shape Expressions (ShEx) and Shapes Constraint Language (SHACL). In this paper we describe how these formalisms can be used in the development of a linked data portal to describe and validate its contents. As a use case, we specify a data model inspired by the WebIndex data model, a medium size linked data portal, using both ShEx and SHACL, and we propose a benchmark that can generate compliant test data structures of any size. We then perform some preliminary experiments showing performance of one validation engine based on ShEx.

==> annexSHACL.tex <==
\clearpage
\section{Annex II: Webindex Schema in SHACL}
\label{SHACL Shapes}

\begin{lstlisting}[style=Turtle]
@prefix : <http://example.org/> .
@prefix sh: <http://www.w3.org/ns/shacl#> .
@prefix xsd: <http://www.w3.org/2001/XMLSchema#> .
@prefix rdf: <http://www.w3.org/1999/02/22-rdf-syntax-ns#>.
@prefix wf: <http://data.webfoundation.org#>.
@prefix rdfs: <http://www.w3.org/2000/01/rdf-schema#>.
@prefix qb: <http://purl.org/linked-data/cube#> .
@prefix cex: <http://purl.org/weso/ontology/computex#> .
@prefix dct: <http://purl.org/dc/terms/>.
@prefix skos: <http://www.w3.org/2004/02/skos/core#>.
@prefix foaf: <http://xmlns.com/foaf/0.1/> .
@prefix org: <http://www.w3.org/ns/org#> .


:Country a sh:Shape ;
 sh:property [
	  sh:predicate rdfs:label ;
	  sh:datatype xsd:string ;
	  sh:minCount 1 ; sh:maxCount 1 ;
	] ;
 sh:property [
	  sh:predicate wf:iso2 ;
	  sh:datatype xsd:string ;
	  sh:minCount 1 ; sh:maxCount 1 ;
	].

:DataSet a sh:Shape ;
 sh:property [
	  sh:predicate rdf:type ;
	  sh:hasValue qb:DataSet ;
	  sh:minCount 1 ; sh:maxCount 1 ;
	] ;
 sh:property [
	  sh:predicate qb:structure ;
	  sh:hasValue wf:DSD ;
	  sh:minCount 1 ; sh:maxCount 1 ;
	] ;
 sh:property [
	  sh:predicate rdfs:label ;
	  sh:datatype xsd:string ;
	  sh:minCount 0 ; sh:maxCount 1 ;
	] ;
 sh:property [
	  sh:predicate qb:slice ;
	  sh:valueShape :Slice ;
	  sh:minCount 0 ;
	] ;
 sh:property [
	  sh:predicate dct:publisher ;
	  sh:valueShape :Organization ;
	  sh:minCount 1; sh:maxCount 1 ;
	] ;
.

:Slice a sh:Shape ;
 sh:property [
	  sh:predicate rdf:type ;
	  sh:hasValue qb:Slice ;
	  sh:minCount 1; sh:maxCount 1 ;
	] ;
 sh:property [
	  sh:predicate qb:sliceStructure ;
	  sh:hasValue wf:sliceByYear ;
	  sh:minCount 1; sh:maxCount 1 ;
	] ;
 sh:property [
	  sh:predicate qb:observation ;
	  sh:valueShape :Observation ;
	  sh:minCount 0;
	] ;
 sh:property [
	  sh:predicate cex:indicator ;
	  sh:valueShape :Indicator ;
	  sh:minCount 1; sh:maxCount 1 ;
	] ;
.

:Observation a sh:Shape ;
	sh:property [
		sh:predicate rdf:type ;
		sh:qualifiedMinCount 1 ;
		sh:qualifiedValueShape [
			sh:constraint [ sh:in ( qb:Observation ) ]
		] ;
	] ;
	sh:property [
		sh:predicate rdf:type ;
		sh:qualifiedMinCount 1 ;
		sh:qualifiedValueShape [
			sh:constraint [ sh:in ( wf:Observation ) ]
		] ;
	] ;
	sh:property [
	   sh:predicate rdf:type ;
	   sh:minCount 2 ; sh:maxCount 2
	] ;
 sh:property [
	  sh:predicate cex:value ;
	  sh:datatype xsd:float ;
	  sh:minCount 1 ; sh:maxCount 1
	] ;
 sh:property [
	  sh:predicate rdfs:label ;
	  sh:datatype xsd:string ;
	  sh:minCount 0; sh:maxCount 1
	] ;
 sh:property [
	  sh:predicate dct:issued ;
	  sh:datatype xsd:dateTime ;
	  sh:minCount 1; sh:maxCount 1
	] ;
 sh:property [
        sh:predicate dct:publisher ;
        sh:hasValue wf:WebFoundation ;
        sh:filterShape [
            sh:property [
                sh:predicate dct:publisher ;
                sh:minCount 1 ;
            ]
        ] ;        
        sh:maxCount 1 ;
    ] ;	
 sh:property [
	  sh:predicate qb:dataSet ;
	  sh:valueShape :DataSet ;
	  sh:minCount 1 ; sh:maxCount 1
	] ;
 sh:property [
	  sh:predicate cex:ref-area ;
	  sh:valueShape :Country ;
	  sh:minCount 1; sh:maxCount 1
	] ;
 sh:property [
	  sh:predicate cex:indicator;
	  sh:valueShape :Indicator ;
	  sh:minCount 1; sh:maxCount 1
	] ;	
 sh:property [
	  sh:predicate cex:ref-year ;
	  sh:datatype xsd:gYear ;
	  sh:minCount 1; sh:maxCount 1
	] ;
 sh:constraint [
 a sh:OrConstraint ;
 sh:shapes (
	[ sh:property [
	  sh:predicate wf:source ;
	  sh:nodeKind sh:IRI ;
	  sh:minCount 1; sh:maxCount 1 ;
	]]
	[ sh:property [
	  sh:predicate cex:computation ;
	  sh:valueShape :Computation ;
	  sh:minCount 1; sh:maxCount 1 ;
	]]
  ) 
 ] ;
 sh:constraint [
  a sh:NotConstraint ;
  sh:shape [ 
  sh:constraint [
  a sh:AndConstraint ;
  sh:shapes (
   [ sh:property [
	  sh:predicate wf:source ;
	  sh:nodeKind sh:IRI ;
	  sh:minCount 1; sh:maxCount 1 
   ]]
   [ sh:property [
	  sh:predicate cex:computation ;
	  sh:valueShape :Computation ;
	  sh:minCount 1; sh:maxCount 1 ;
	]] )
 ]]] .	

:Computation a sh:Shape ;
 sh:property [
  sh:predicate rdf:type ;
  sh:hasValue cex:Computation ;
  sh:minCount 1; sh:maxCount 1
 ].

:Indicator a sh:Shape ;
 sh:property [
	  sh:predicate rdf:type ;
	  sh:in (
	     wf:PrimaryIndicator 
	     wf:SecondaryIndicator
	  ) ;
	  sh:minCount 1; sh:maxCount 1 ;
	] ; 
 sh:property [
	  sh:predicate rdfs:label ;
	  sh:datatype xsd:string ;
	  sh:minCount 1; sh:maxCount 1 ;
	] ; 
 sh:property [
	  sh:predicate wf:provider ;
	  sh:valueShape :Organization ;
	  sh:minCount 1; sh:maxCount 1 ;
	].	
	
:Organization a sh:Shape ;
  sh:constraint [
   a sh:ClosedShapeConstraint;
   sh:ignoredProperties(rdf:type)
  ] ;
 sh:property [
  sh:predicate rdf:type ;
  sh:hasValue org:Organization ;
 ] ;
 sh:property [
  sh:predicate rdfs:label ;
  sh:datatype xsd:string ;
  sh:minCount 1; sh:maxCount 1 ;
 ] ;
 sh:property [
  sh:predicate foaf:homepage ;
  sh:nodeKind sh:IRI ;
  sh:minCount 1; sh:maxCount 1 ;
] .
\end{lstlisting}


==> annexShEx.tex <==
\clearpage
\section{Annex I: WebIndex Schema in ShEx}

\begin{lstlisting}[style=ShExC]
prefix : <http://example.org/> 
prefix sh: <http://www.w3.org/ns/shacl#> 
prefix xsd: <http://www.w3.org/2001/XMLSchema#> 
prefix rdf: <http://www.w3.org/1999/02/22-rdf-syntax-ns#>
prefix wf: <http://data.webfoundation.org#>
prefix rdfs: <http://www.w3.org/2000/01/rdf-schema#>
prefix qb: <http://purl.org/linked-data/cube#> 
prefix cex: <http://purl.org/weso/ontology/computex#> 
prefix dct: <http://purl.org/dc/terms/>
prefix skos: <http://www.w3.org/2004/02/skos/core#>
prefix foaf: <http://xmlns.com/foaf/0.1/>
prefix org: <http://www.w3.org/ns/org#>

:Country {
  rdfs:label        xsd:string, 
  wf:iso2           xsd:string
}
:DataSet { a        (qb:DataSet), 
  qb:structure      (wf:DSD),
  rdfs:label        xsd:string, 
  qb:slice          @:Slice*, 
  dct:publisher     @:Organization
}
:Slice { a          (qb:Slice), 
  qb:sliceStructure (wf:sliceByYear),
  qb:observation    @:Observation*, 
  cex:indicator     @:Indicator
}
:Observation { a    (qb:Observation), 
  a                 (wf:Observation), 
  cex:value         xsd:float,
  rdfs:label        xsd:string?,
  dct:issued        xsd:dateTime, 
  dct:publisher     (wf:WebFoundation)?, 
  qb:dataSet        @:DataSet, 
  cex:ref-area      @:Country, 
  cex:indicator     @:Indicator, 
  cex:ref-year      xsd:gYear, 
  ( cex:computation @:Computation 
  | wf:source       IRI 
  )
}
:Computation { a    (cex:Computation) }

:Indicator { a      (wf:PrimaryIndicator wf:SecondaryIndicator), 
 rdfs:label        xsd:string, 
 wf:provider       @:Organization
}
:Organization CLOSED EXTRA a { a (org:Organization), 
 rdfs:label        xsd:string, 
 foaf:homepage     IRI
}
\end{lstlisting}


